CGELBank: CGEL as a Framework for English Syntax Annotation

We introduce the syntactic formalism of the \textit{Cambridge Grammar of the English Language} (CGEL) to the world of treebanking through the CGELBank project. We discuss some issues in linguistic analysis that arose in adapting the formalism to corpus annotation, followed by quantitative and qualitative comparisons with parallel UD and PTB treebanks. We argue that CGEL provides a good tradeoff between comprehensiveness of analysis and usability for annotation, which motivates expanding the treebank with automatic conversion in the future.

==> old-counts.tex <==
\begin{table}
    \centering\small
    \setlength{\tabcolsep}{2.5pt}
    \adjustbox{max width=\columnwidth}{
    \begin{tabular}{rl rl rl}
    \toprule
    \multicolumn{2}{c}{\textbf{POS}} & \multicolumn{2}{c}{\textbf{Phrasal Category}} & \multicolumn{2}{c}{\textbf{Gram.~Function}} \\
    \cmidrule(r){1-2}\cmidrule(r){3-4}\cmidrule{5-6}
    %%%% produced by analysis/cgel_pos.py
680 & N           & 1232 & Nom                  & 2082 & \func{Head} \\
583 & V           &  893 & NP                   &  606 & \func{Mod} \\
323 & P           &  756 & VP                   &  401 & \func{Comp} \\
311 & D           &  632 & Clause               &  390 & \func{Obj} \\
255 & N\textsubscript{pro}      &  334 & PP                   &  301 & \func{Subj} \\
170 & Adj         &  307 & DP                   &  297 & \func{Det} \\
129 & Adv         &  183 & AdjP                 &  211 & \func{Coordinate} \\
102 & Sdr         &  130 & AdvP                 &   87 & \func{PredComp} \\
100 & Coordinator &   81 & Coordination         &   67 & \func{Supplement} \\
  2 & Int         &   50 & Clause\textsubscript{rel}          &   58 & \func{Det-Head} \\
    &             &   29 & Flat*                 &   28 & \func{Prenucleus} \\
84 & \textit{GAP}             &    7 & MultiSentence*        &    8 & \func{ExtraposedSubj} \\


    % &             &    6 & Clausal-coordination &    7 & Particle \\
    % &             &    6 & NP+PP                &    7 & Postnucleus \\
    % &             &    3 & V                    &    6 & Obj\_dir \\
    % &             &    2 & Clausal-Coordination &    6 & Obj\_ind \\
    % &             &    2 & NP+Clause            &    4 & Head-Prenucleus \\
    % &             &    1 & NP+VP Coordination   &    4 & DisplacedSubj \\
    % &             &    1 & NP-Coordination      &    3 & Vocative \\
    % &             &    1 & VP-Coordination      &    3 & Comp\_ind \\
    % &             &    1 & VP-coordination      &    3 & Mod-Head \\
    % &             &    1 & Clausal Coordination &    2 & PreDetMod \\
    % &             &    1 & Emoji                &    1 & Head-Subject \\
    % &             &    1 & ClausalCoordination  &    1 & Obj+PredComp/Comp \\
    % &             &    1 & Supplement           &      &  \\
    % &             &    1 & NP-coordination      &      &  \\
    % &             &    1 & NP+AdjP              &      &  \\
        \bottomrule
    \end{tabular}}
    \caption{Counts in CGELBank POS tags, phrasal categories, and grammatical functions. Special phrasal categories for coordination and some functions are not listed due to low frequency.\\
    % \br{Can we strike this second sentence and rely on the note below?}\nss{I guess it was unclear---it referred to things omitted. Maybe: ``There are also infrequent phrasal categories due to coordination.'' Or change the first sentence to ``phrasal categories occurring 7 or more times''. I put extra table rows in a comment showing what was omitted}
    *\, Dummy categories to ensure token- and tree-level alignment with UD.}
    %Infrequent grammatical functions are: ExtraposedSubj, Particle, Postnucleus, Obj\_dir, Obj\_ind, Head-Prenucleus, DisplacedSubj, Modifier-Head, PreDetMod, Vocative, Head-Subject, Head-Comp, Comp\_ind, and Obj~+~PredComp/Comp [due to gapping].
    % \br{what's "multiSentence \& sentence?}\nss{when two sentences are basically glued together i think}\br{but the trees never have something called "sentence". The root node is typically \textit{clause}, which is a phrasal category, not a function.}\nss{Right, MultiSentence/:Sentence is just a technical way to bring together two trees. E.g. ``ItIsntThat.pdf'' in the Twitter data is annotated as 2 trees. Because we want a single root for computational reasons}
    % \br{OK, I can see ``MultiSentence'', but ``Sentence'' can't possibly be a function, can it? And ``Flat'' and ``MultiSentence'' can't be ``phrasal categories'' because phrases have heads. Can we have ``Lexical Categories'' instead of POS (throughout as it applies to CGEL at least?), and add ``Flat'' and ``MultiSentence'' in a note or something?}
    \label{tab:catcounts}
\end{table}

